ROPfuscator: Robust Obfuscation with ROP

Software obfuscation plays a crucial role in protecting intellectual property in software from reverse engineering attempts. While some obfuscation techniques originate from the obfuscation-reverse engineering arms race, others stem from different research areas, such as binary software exploitation. Return-oriented programming (ROP) gained popularity as one of the most effective exploitation techniques for memory error vulnerabilities. ROP interferes with our natural perception of a process control flow, inspiring us to repurpose ROP as a robust and effective form of software obfuscation. Although previous work already explores ROP's effectiveness as an obfuscation technique, evolving reverse engineering research raises the need for principled reasoning to understand the strengths and limitations of ROP-based mechanisms against man-at-the-end (MATE) attacks. To this end, we present ROPfuscator, a compiler-driven obfuscation pass based on ROP for any programming language supported by LLVM. We incorporate opaque predicates and constants and a novel instruction hiding technique to withstand sophisticated MATE attacks. More importantly, we introduce a realistic and unified threat model to thoroughly evaluate ROPfuscator and provide principled reasoning on ROP-based obfuscation techniques that answer to code coverage, incurred overhead, correctness, robustness, and practicality challenges.

==> latexmkrc <==
# Settings
$xdvipdfmx = "xdvipdfmx -z 6 -o %D %O %S";

###############################
# Post processing of pdf file #
###############################

# assume the jobname is 'output' for sharelatex
my $ORIG_PDF_AGE = -M "output.pdf"; # get age of existing pdf if present

END {
    my $NEW_PDF_AGE = -M "output.pdf";
    return if !defined($NEW_PDF_AGE); # bail out if no pdf file
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE; # bail out if pdf was not updated
    $qpdf //= "/usr/local/bin/qpdf";
    $qpdf = $ENV{QPDF} if defined($ENV{QPDF}) && -x $ENV{QPDF};
    return if ! -x $qpdf; # check that qpdf exists
    $qpdf_opts //= "--linearize --newline-before-endstream";
    $qpdf_opts = $ENV{QPDF_OPTS} if defined($ENV{QPDF_OPTS});
    my $status = system($qpdf, split(' ', $qpdf_opts), "output.pdf", "output.pdf.opt");
    my $exitcode = ($status >> 8);
    print "qpdf exit code=$exitcode\n";
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($exitcode == 0 || $exitcode == 3);
    print "Renaming optimised file to output.pdf\n";
    rename("output.pdf.opt", "output.pdf");
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
    system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
    $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
        system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
my $root_file = $ARGV[-1];

add_cus_dep( 'Rtex', 'tex', 0, 'rtex_to_tex');
sub rtex_to_tex {
    do_knitr("$_[0].Rtex");
}

sub do_knitr {
    my $dirname = dirname $_[0];
    my $basename = basename $_[0];
    system("Rscript -e \"library('knitr'); setwd('$dirname'); knit('$basename')\"");
}

my $rtex_file = $root_file =~ s/\.tex$/.Rtex/r;
unless (-e $root_file) {
    if (-e $rtex_file) {
        do_knitr($rtex_file);
    }
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############
sub asy {return system("asy --offscreen '$_[0]'");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
    my $file = $_[0];
    my ($name, $path) = fileparse($file);
    pushd($path);
    my $return = system "mpost $name";
    popd();
    return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
        # change directory for a limited scope
        my $orig_dir = cwd();
        my $subdir = dirname($target);
        chdir($subdir);
        # run chktex on main file
        $status = system("/usr/bin/run-chktex.sh", $orig_dir, $file);
        # go back to original directory
        chdir($orig_dir);

        # in VALIDATE mode we always exit after running chktex
        # otherwise we exit if EXIT_ON_ERROR is set

        if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
            # chktex doesn't let us access the error info via exit status
            # so look through the output
            open(my $fh, "<", "output.chktex");
            my $errors = 0;
            {
                local $/ = "\n";
                while(<$fh>) {
                    if (/^\S+:\d+:\d+: Error:/) {
                        $errors++;
                        print;
                    }
                }
            }
            close($fh);
            exit(1) if $errors > 0;
            exit(0) if $ENV{'CHKTEX_VALIDATE'};
        }
    }
}

==> sec-background.tex <==
\section{Background}
\label{sec:background}

In this section, we introduce return-oriented programming which is used as a basis of our obfuscation scheme (\S\ref{subsec:background:rop}), as well as other software obfuscation techniques which are incorporated into our approach (\S\ref{subsec:background:obfuscation}). Finally, we describe reverse engineering techniques considered in the threat model (\S\ref{subsec:background:reversing}).

\subsection{Return Oriented Programming}
\label{subsec:background:rop}

Return oriented programming (ROP), is a binary exploitation technique which reuses existing code in programs to execute arbitrary algorithms \cite{shacham_geometry_2007, roemer_return-oriented_2012}.

Code written using ROP is called \textit{rop chain} and it is composed of \textit{gadgets}, a sequence of instructions followed by a final return instruction.

\begin{figure}
	\centering
	\footnotesize
	\newsavebox{\boxrightarrow}
	\sbox{\boxrightarrow}{
		\begin{tikzpicture}[x=0.1em,y=0.1em]
			\draw (0,5)--(0,15)--(10,15)--(10,20)--(20,10)--(10,0)--(10,5)--cycle;
		\end{tikzpicture}
	}
	\begin{tikzpicture}[x=0.12em,y=0.12em]
		\draw (30,0)--(30,70)--(80,70)--(80,0)
		(30,60)--(80,60)
		(30,40)--(80,40)
		(30,30)--(80,30)
		(30,20)--(80,20)
		(30,10)--(80,10);
		\node at (55,80){\textsf{stack}};
		\node at (55,65){local vars};
		\node at (55,55){\texttt{buf}};
		\node at (55,45){\dots};
		\node at (55,35){return addr};
		\node at (55,25){arg1};
		\node at (55,15){arg2};
		\node at (95,35){\usebox{\boxrightarrow}};
		\fill[black!15] (110,0)--(110,60)--(160,60)--(160,0)--cycle;
		\draw (110,0)--(110,70)--(160,70)--(160,0)
		(110,60)--(160,60)
		(110,40)--(160,40)
		(110,30)--(160,30)
		(110,20)--(160,20)
		(110,10)--(160,10);
		\node at (135,80){\textsf{stack with ROP chain}};
		\node at (135,65){local vars};
		\node at (135,55){\texttt{AAAAAAAA}};
		\node at (135,45){\texttt{AAAAAAAA}};
		\node at (135,35){\texttt{0x40123}};
		\node at (135,25){\texttt{0x40456}};
		\node at (135,15){\texttt{1234}};
		\node at (135,5){\dots};
		\filldraw[color=black,fill=black!15] (190,60)--(260,60)--(260,40)--(190,40)--cycle;
		\filldraw[color=black,fill=black!15] (190,30)--(260,30)--(260,10)--(190,10)--cycle;
		\draw (190,0)--(190,70) (260,0)--(260,70);
		\draw[->] (165,35)--(185,55);
		\draw[dashed,->] (185,45)--(165,27);
		\draw[->] (165,25)--(185,25);
		\draw[dashed,->] (185,15)--(165,7);
		\node at (225,80){\textsf{code memory}};
		\node[anchor=west] at (260,60){\scriptsize\texttt{0x40123}};
		\node[anchor=west] at (260,30){\scriptsize\texttt{0x40456}};
		\node[text width=7em] at (225,50){\texttt{xchg eax,ecx \\ ret}};
		\node[text width=7em] at (225,20){\texttt{pop ecx \\ ret}};
	\end{tikzpicture}
	\caption{ROP chain execution on the stack}
	\label{fig:rop}
\end{figure}


When ROP is used to exploit a program, the rop chains are usually injected through a buffer overflow vulnerability to control the instruction pointer. We explain the execution of a rop chain in an example detailed in Figure. \ref{fig:rop} which considers the attack being executed onto the stack.

In this example, the gadget \Code{xchg eax, ecx; ret} located at address \Code{0x40123} exchanges registers \Code{eax} and \Code{ecx}. When the \Code{ret} instruction is executed, the return address \Code{0x40456} is popped from the stack and set as new instruction pointer; the chain is now executing its second gadget that pops \Code{ecx} from the stack. By carefully choosing available gadgets in the target binary, an attacker can execute arbitrary code (e.g. spawning a shell).

ROP is used to bypass a binary with a non-executable memory region ($\mathrm{W}\oplus\mathrm{X}$) or to hide attack vectors.


\subsection{Software Obfuscation}
\label{subsec:background:obfuscation}

Software obfuscation is the process of altering a program with added complexity without changing its functionality \cite{aucsmith_tamper_1996, wang_protection_2001, linn_obfuscation_2003}. While it is theoretically impossible to obfuscate software in such a way as to revert it to an intelligible form \cite{barak_impossibility_2001}, there are commercial products and academic studies that explored the different ways to obfuscate programs. Dummy code insertion, control flow flattening, self-modifying code and virtualization are some of the most used obfuscation techniques.

\textit{Dummy, or junk, code insertion} \cite{linn_obfuscation_2003} consists in the insertion of semantically useless instructions to confuse static analysis and to prevent a disassembler from correctly disassembling the code.


\textit{Control flow flattening} \cite{chow_approach_2001} deconstructs a control flow graph into disconnected instruction blocks subsequently invoked in the proper order by a central dispatcher, which keeps track of the state of the execution.

\textit{Self-modifying code} \cite{kanzaki_exploiting_2003} is a portion of code that will overwrite itself at run-time, vastly differentiating from its compile-time version. It effectively hides instructions from static analysis, although it imposes a significant performance loss due to instruction caching.

\textit{Virtualization-based obfuscation} \cite{anckaert_proteus_2006} consists in compiling code for an emulated CPU target whose instructions may not reflect any other real-life examples.The complexity of the instruction set of the emulated CPU spans from a copycat of existing architectures to esoteric ones.

In this paper, we focus on opaque predicates and opaque constants and their use combined with dummy code insertion.

\paragraph{Opaque Predicates and Opaque Constants}

An \emph{opaque predicate} \cite{collberg_manufacturing_1998} is a function that maps all its inputs to a single-bit constant output, true (\Code{1}) or false (\Code{0}). These predicates' characteristic is the complex relationship between their input and output, often based on mathematical problems. 3-SAT, a subset of the Boolean Satisfiability Problem known to be NP-hard, is one of the most used approaches in generating opaque predicates \cite{moser_limits_2007, sheridan_manufacturing_2016}.

There are three main types of opaque predicates documented in literature: invariant, contextual, and dynamic opaque predicates. \textit{Invariant} opaque predicates always evaluate to the same value, decided a-priori by the obfuscator. \textit{Contextual} opaque predicates change their output based on preconditions chosen at design-time \cite{drape_intellectual_2010}. \textit{Dynamic} opaque predicates introduce the idea of correlated predicates that maps the output of a predicate to the input of a subsequent one \cite{palsberg_experience_2000}.

Additionally, opaque predicates are used to obfuscate control flow and value generation to protect dummy code blocks that are never executed.

\textit{Opaque constants} \cite{moser_limits_2007} are used to generate arbitrary values by combining the output bit, where the program branches based on the predicate output and the conditional branches to those blocks will never be executed of several opaque predicates together. Opaque constants can be used to obfuscate meaningful immediate values in applications such as jump target addresses, cryptographic constants, and immediate operands.

\subsection{Software Reverse Engineering}
\label{subsec:background:reversing}

Software reverse engineering is the analysis of a program when its source code is not available. It is applied to data objects whose format is designed to be processed by a machine rather than a human (e.g., a compiled executable). Due to the complexity of recovering intelligible information from data optimized for machine consumption, reverse engineering is a tedious and error-prone task for human analysts. Therefore, different tools, algorithms, and techniques have been developed to ease this process.

\paragraph{Static analysis}

Static analysis is the process of studying a program without executing it. It provides high-quality information and prevents potentially malicious code from being executed during the analysis. However, this might not be time-efficient, depending on the size of the application to study.

A \textit{disassembler} is a fundamental static analysis tool. It translates binary machine code into human-readable form, namely, assembly code. The most common disassembly algorithms are linear sweep and recursive traversal \cite{schwarz_disassembly_2002}. \textit{Linear sweep} disassembles a binary blob from an arbitrary starting location until it reaches an illegal instruction: this is a swift yet fragile approach due to the lack of further analysis of the disassembled code. \textit{Recursive traversal}, on the other hand, extends linear sweep to take into account control flow instructions such as \Code{call}, \Code{ret} or \Code{jmp}, identifying additional code locations for further processing.

Once a program is disassembled, its output may be processed further by a \textit{decompiler}. It applies heuristics and several analyses to retrieve a high-level representation compared to pseudocode for easier understanding.


\paragraph{Dynamic analysis and symbolic execution}

\textit{Dynamic analysis} is opposed to static analysis and focuses on observing a program's behavior during its execution. This allows the analyst to gather a rough understanding of the application quickly. However, this can result in missing events triggered on specific occasions or inputs. For this reason, a combination of static and dynamic analysis usually provides better results.

\textit{Dynamic symbolic execution} (DSE) is a technique to simulate the execution of programs \cite{godefroid_dart_2005, sen_cute_2005}. Evolved from symbolic execution \cite{king_symbolic_1976}, DSE is also known as \textit{concolic execution} since it executes programs both \emph{conc}retely, (i.e., using values obtained from the running program) and symb\emph{olic}ally (i.e., using variables for values that are unknown at run-time).


DSE efficiently explores control flow graphs to discover branches activated by specific events or input values \cite{ollivier_how_2019}. Simultaneously, researchers have developed attacks against concolic execution, which exploits the weaknesses inherited from SMT solvers' usage (e.g., execution path explosion) \cite{banescu_code_2016, xu_manufacturing_2018, ollivier_how_2019}.

\paragraph{ROP specific analysis}

ROP is mainly used as a binary exploitation technique to gain arbitrary code execution. Researchers have proposed different approaches to analyze and mitigate it. We consider the following studies as benchmarks for our proposed obfuscation methodology.

\textit{deRop} \cite{lu_derop_2011} proposes a static analysis technique to transform ROP chains into linear assembly. It traverses a ROP chain and locates its gadget addresses to extract and recover the original code finally.

\textit{ROPMEMU} \cite{graziano_ropmemu_2016} is a malware analysis framework with dynamic tracing capabilities on memory dumps. It features multi-path emulation to extract the ROP chains, control flow graph recovery, and compiler optimizations to simplify and rebuild the initial code.

\textit{ROPdissector} \cite{delia_static_2019} is an emulation-based analysis framework that allows the dissection and emulation of ROP gadgets without requiring context information in which the ROP chain has to be executed.
